LEASGD: an Efficient and Privacy-Preserving Decentralized Algorithm for Distributed Learning

Distributed learning systems have enabled training large-scale models over large amount of data in significantly shorter time. In this paper, we focus on decentralized distributed deep learning systems and aim to achieve differential privacy with good convergence rate and low communication cost. To achieve this goal, we propose a new learning algorithm LEASGD (Leader-Follower Elastic Averaging Stochastic Gradient Descent), which is driven by a novel Leader-Follower topology and a differential privacy model.We provide a theoretical analysis of the convergence rate and the trade-off between the performance and privacy in the private setting.The experimental results show that LEASGD outperforms state-of-the-art decentralized learning algorithm DPSGD by achieving steadily lower loss within the same iterations and by reducing the communication cost by 30%. In addition, LEASGD spends less differential privacy budget and has higher final accuracy result than DPSGD under private setting.

==> 2_Background.tex <==
\section{Related Work}
\label{sec:back}
Quantization is one of the ways to make the existing neural networks deployable on platforms with a limited computational/memory/power resource. This process usually involves a scaling operation, where the float weights are rescaled to integer numbers with a float scaling factor. Previous researchers have explore different methods of quantization as mentioned below.

For example, Intel(R) introduced MKL-DNN\cite{b5} as a toolset which converts the 32-bit float weights to 8-bit integers with only tolerable accuracy loss. The weights in the same layer have a shared scale factor λ which converts the original float weights to quantized integers, as well as the biases and input data from the previous layer. Therefore, the operation of the float data can be done by multiplying the result of the same operation on the quantized integer data by the overall scale factor. NVIDIA's TensorRT\cite{b6} is based on the same scheme with more complicated choice of scale factor which takes into both the granularity and information loss into consideration. 

MatthieuCourbariaux et al.\cite{b1} exploits the above idea with a more radical binary representation of all the inputs,  weights and activations. Furthermore, it takes the advantage of binary representation by incorporating several optimization algorithms which conducts the normal operation such as multiplication, batch normalization and Adam Optimization in a bitwise manor, thus even achieving higher computation efficiency. Rastegari et al.\cite{b2} proposed a more theoretical analysis on the binary network and introduced scale factor in their XNOR-Net, a network based on MatthieuCourbariaux et al.\cite{b1} with much higher accuracy. Despite significant speedup on inference, neither of the above network have been reported to achieve comparable accuracy as the full-precision ones, thus preventing binary neural network from being deployed in real-world application.


==> 7_Conclusion.tex <==
\section{Conclusion} %and Future work}
\label{sec:con}

In this paper, we propose a new decentralized algorithm \LEASGD for training deep neural network with differential privacy.
%distributed datasets and also design a  specific scheme for it to implement in a privacy-sensitive setting. 
\LEASGD ensures differential privacy with improved convergence rate and communication efficiency, thanks to the novel leader-follower protocol and privacy-preserving schemes.  
We theoretically prove its exponential decreasing convergence rate as a function of iterations and good scalability.
We also provide a thorough analysis of the performance and privacy trade-off. 
The real distributed testbed evaluation results show \LEASGD outperforms the state-of-the-art decentralized learning algorithm DPSGD in both convergence rate and privacy budget.
with faster convergence rate under the same iterations and communication cost.
In addition, \LEASGD achieves higher accuracy as DPSGD with less spent privacy budget in the private setting.
adopting our \LEASGD algorithm. Also, it achieves the same accuracy as DPSGD with less spent privacy budget in the private setting.

%Further research is needed to implement our algorithm into a multi-GPU system and communication network with different bandwidth and thus to count the wall clock time to evaluate our algorithm and compare with others more accurately. In this way, we can also implement asynchronous version of our algorithm that is closed to real-life application. 



==> 9_supplementary_material.tex <==
\section{Supplementary Material}
\subsection{Algorithm 1}
\begin{algorithm}[]
\caption{Synchronous Follower Elastic Averaging Stochastic Gradient Descent Gradient Descent}
\begin{algorithmic}[1]
\STATE {\textbf{Require:}} initial parameter vectors $w_0^i$, the number of workers $m$, the number of followers $L$, categorization interval $k$, communication interval $\tau$, elastic factor $\rho$, learning rate $\eta$
\STATE \FOR{\textbf{$iteration t=1,2,......,T$}}
\STATE \IF {\textbf{$t\ mod\ k\tau\ is\ 0$}}
\STATE \IF {\textbf{$t\ =\ 0$}}
\STATE randomly select $L$ followers $l_1,......,l_L$
\STATE \ELSE 
\STATE sort the loss function value and categorize $L$ followers
\STATE $\ \ \ \ {l_1,......,l_L}= \mathop{argmaxL}\limits_{i=1,...,m}f^i_t(\omega^i)$
\ENDIF
\ENDIF
\STATE \IF{$t\ mod\ \tau\ is\ 0$}
\STATE \FOR{\textbf{followers:}$i\in \{l_1,......,l_L\}$}
\STATE  local SGD updating
\ENDFOR
\STATE \FOR{\textbf{ followers:$i\notin \{l_1,......,l_L\}$}}
\STATE randomly select a follower $f$ from follower pool
\STATE transmit parameter vectors with $f$ and do elastic updating
\ENDFOR
\STATE \ELSE
\STATE \FOR{\textbf{all workers: }$i\in \{1,......,m\}$}
\STATE  local SGD updating
\ENDFOR
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}



\subsection{Detail Proof of Proposition 1}
Before we show the result of the convergence rate, we first introduce some assumptions held in the analysis.
\newtheorem{assumption}{Assumption}%[section]
\begin{assumption}\label{ass:ass1}

These assumptions are held throughout the analysis:\\
1. \textbf{i.i.d. assumption}: We divide our system into several sub-systems with only 1 follower and $p$ leaders. And all the variables in these sub-systems are i.i.d.\\
2. \textbf{Correct categorization}: Assume that since the categorization step in Algorithm 1 is implemented, the identity of all workers will not change until the next categorization\\
3. \textbf{Bounded stochastic gradient}: Assume that the variance of all the local gradients is bounded for any $w$ for any workers from ${1,...,m}$ and input $x^i_t$. There exist constant $\sigma_1$ such that \begin{equation}
    \label{bound_gradient}
    \begin{split}
        E[g^i_t-\bigtriangledown f(w^i_t)]=0\ and\\
        E[\parallel g^i_t-\bigtriangledown f(w^i_t)\parallel^2]\le\sigma_1^2
    \end{split}
\end{equation}
4. \textbf{Strongly convex condition}: We only discuss about the strongly-convex case in the analysis. Correspondlingly, there exists $0<\mu\le L$ for all the loss functions:

\begin{equation}
    \label{regularized_function}
    %\begin{split}
        f^i_{t}(w^i)=l(w^i_t,x^i_t,y^i_t)+\lambda\parallel w^i\parallel_2
    %\end{split}
\end{equation}

and we can rewrite it to:

\vspace{-7mm}

\begin{equation}
    \label{strongly_convex}
    \begin{split}
        \mu \parallel w_i-w_j \parallel ^2 \le \langle\bigtriangledown f(w_i),\bigtriangledown f(w_j)\rangle\le L\parallel w_i-w_j \parallel ^2
    \end{split}
\end{equation}
\end{assumption}

\vspace{-6mm}

We define that
\begin{equation}
    \label{d_t}
    \begin{split}
        d_t=\frac{E\sum_{i=1}^{p}\parallel w^i_t-w^*\parallel^2+E\parallel w^f_t-w^*\parallel^2}{p+1}
    \end{split}
\end{equation}

\vspace{-3mm}

and under Assumption \ref{ass:ass1}, we can obtain the result of convergence rate of $d_t$ in Algorithm 1


We first provide the proof of convergence rate of Algorithm 1 under a strongly-convex case. In the analysis, we mainly focused on the average square of the distance between all workers to the optimum, that is $d_t$ shown in the proposition. We draw the ideas from the convergence analysis of EASGD under a strongly-convex case \cite{zhang2015deep} but further specify it to our algorithm. Under the first assumption in Assumption \ref{ass:ass1}, we simplify our system by dividing it into several subsystems and each includes only 1 follower and $p$ leaders. We assume that the convergence rate of each subsystem is the same as that of the whole system. 

To obtain this convergence rate, we will need following theorem.
\begin{mytheo}
Let $y_t= \frac{1}{p}\sum_{i=1}^{p} w^i_t$, $a_t=E\parallel y_t-w^*\parallel^2$, $b_t=\frac{1}{p}\sum_{i=1}^{p}E\parallel w^i_t-w^*\parallel^2$, $c_t=E\parallel w^f_t-w^*\parallel^2$, $\alpha=\eta\rho$, $\beta=p\alpha$,$\gamma=2\eta\frac{\mu L}{\mu+L}$. If $0\le\eta\le\frac{2(1-\beta)}{\mu+L}$,$0\le\alpha<1$,$0\le\beta<1$, then
\begin{align}
    b_{t+1}\le(1-\gamma-\alpha)b_t+\alpha c_t+\eta^2\sigma_1^2\\
    c_{t+1}\le(1-\gamma-\beta)c_t+\beta a_t+\eta^2\sigma_1^2
\end{align}
\end{mytheo}

\emph{Proof}
Under the third assumption of Assumption \ref{ass:ass1}, the noisy gradient $g_t^i$ of all the workers can be rewritten as $g_t^i=\bigtriangledown f(w^i_t)+\xi_t^i$ in which $E[\xi_t^i]=0$ and $E\parallel \xi_t^i\parallel^2<\sigma_1^2$. Then the updating rules of Algorithm 1 could be written as
\begin{align}
    w^i_{t+1}=w^i_t-\eta g_t^i-\alpha(w_t^i-w_t^f)\\
    w^f_{t+1}=w^f_t-\eta g_t^f-\beta(w_t^f-y_t)
\end{align}
From equation (3), we have 
\begin{equation}
    \begin{split}
        \parallel w_{t+1}^i-w^*\parallel^2= \parallel w_t-w^*\parallel^2+\eta^2\parallel g_t^i\parallel^2+\alpha^2\parallel w^i_t-w^f_t \parallel^2\\
        -2\eta\langle g_t^i,w^i_t-w^*\rangle-2\alpha \langle w_t^i-w^f_t,w^i_t-w^*\rangle\\+2\eta\alpha\langle g_t^i,w^i_t-w^f_t\rangle
    \end{split}
\end{equation}
By the cosine rule($2\langle a-b,c-d\rangle=\parallel a-d \parallel^2-\parallel a-c \parallel^2+\parallel c-b \parallel^2-\parallel b-d \parallel^2$), we have
\begin{equation}
    \begin{split}
        2\langle w_t^i-w^f_t,w^i_t-w^*\rangle=\parallel w_t^i-w^* \parallel^2+\parallel w^i_t-w^f_t \parallel^2\\
        -\parallel w^f_t-w^* \parallel^2
    \end{split}
\end{equation}

By Cauchy-Schwarz inequality, we have
\begin{equation}
    \begin{split}
        \langle \bigtriangledown f(w^i_t),w^i_t-w^f_t\rangle\le\parallel \bigtriangledown f(w^i_t)\parallel\parallel w^i_t-w^f_t\parallel
    \end{split}
\end{equation}
In the strongly-convex case, we use following theorem of strongly-convex function \cite{nesterov2004introductory}
\begin{equation}
    \begin{split}
        \langle \bigtriangledown F(x)-\bigtriangledown F(y),x-y\rangle\ge\frac{\mu L}{\mu+L}\parallel x-y\parallel^2\\
        +\frac{1}{\mu+L}\parallel \bigtriangledown F(x)-\bigtriangledown F(y)\parallel^2
    \end{split}
\end{equation}
Since $\bigtriangledown f(w^*)=0$, we have
\begin{equation}
    \begin{split}
        \langle \bigtriangledown f(w^i_t),w^i_t-w^*\rangle \ge \frac{\mu L}{\mu+L}\parallel w^i_t-w^*\parallel^2+\frac{1}{\mu+L}\parallel g_t^i\parallel^2
    \end{split}
\end{equation}
Using (5),(6),(7),(9), we thus have
\begin{equation}
    \begin{split}
        \parallel w_{t+1}^i-w^*\parallel^2\le \parallel w_t-w^*\parallel^2+\eta^2\parallel \bigtriangledown f(w^i_t)+\xi^i_t\parallel^2+\alpha^2\parallel w^i_t-w^f_t \parallel^2\\
        -2\eta(\frac{\mu L}{\mu+L}\parallel w^i_t-w^*\parallel^2+\frac{1}{\mu+L}\parallel \bigtriangledown f(w_t^i)\parallel^2)-2\eta\langle \xi^i_t,w^i_t-w^*\rangle\\
        -\alpha(\parallel w_t^i-w^* \parallel^2+\parallel w^i_t-w^f_t \parallel^2-\parallel w^f_t-w^* \parallel^2)\\
        +2\eta\alpha\parallel \bigtriangledown f(w^i_t)\parallel\parallel w^i_t-w^f_t\parallel+2\eta\alpha\langle \xi^i_t,w^i_t-w^f_t\rangle
    \end{split}
\end{equation}
With $0\le\alpha<1$, we bound the term 
\begin{equation}
    \begin{split}
        \alpha^2\parallel w^i_t-w^f_t \parallel^2-\alpha\parallel w^i_t-w^f_t \parallel^2+2\eta\alpha\parallel \bigtriangledown f(w^i_t)\parallel\parallel w^i_t-w^f_t\parallel\\
=\alpha(1-\alpha)\parallel w^i_t-w^f_t \parallel^2+2\eta\alpha\parallel \bigtriangledown f(w^i_t)\parallel\parallel w^i_t-w^f_t\parallel\\
\le\frac{\eta^2\alpha}{1-\alpha}\parallel \bigtriangledown f(w^i_t)\parallel^2
    \end{split}
\end{equation}
by applying $-ax^2+bx\le\frac{b^2}{4a}$ with $x=\parallel w^i_t-w^f_t \parallel^2$. 
Thus, we obtain
\begin{equation}
    \begin{split}
        \parallel w_{t+1}-w^*\parallel^2\le (1-2\eta\frac{\mu L}{\mu+L}-\alpha)\parallel w_t^i-w^*\parallel^2\\
        +(\eta^2+\frac{\eta^2\alpha}{1-\alpha}-\frac{2\eta}{\mu+L})\parallel \bigtriangledown f(w^i_t)\parallel^2+2\eta^2\langle \bigtriangledown f(w^i_t),\xi^i_t\rangle\\
        -2\eta\langle \xi^i_t,w^i_t-w^*\rangle+2\eta\alpha\langle \xi^i_t,w^i_t-w^f_t\rangle
        +\eta^2\parallel \xi^i_t\parallel^2
        \\+\alpha\parallel w^f_t-w^*\parallel^2
    \end{split}
\end{equation}
Given that $E[\xi_t^i]=0$ and $E\parallel \xi_t^i\parallel^2<\sigma_1^2$ and if $\eta$ satisfies $\eta^2+\frac{\eta^2\alpha}{1-\alpha}-\frac{2\eta}{\mu+L}\le0$, then we have
\begin{equation}
    \begin{split}
        E\parallel w_{t+1}-w^*\parallel^2\le(1-2\eta\frac{\mu L}{\mu+L}-\alpha)E\parallel w_t^i-w^*\parallel^2\\
        +\eta^2\sigma^2_1+\alpha\parallel w^f_t-w^*\parallel^2
    \end{split}
\end{equation}
This concludes the proof of (1).
We discover that equation (4) is very similar to the equation (3). If we change
\begin{align}
    w^i_t\to w^i_f\\
    g^i_t\to g^f_t\\
    w^f_t\to y_t\\
    \alpha\to\beta
\end{align}
(3) can be transformed to (4). Thus, we obtain the (2) in the similar way as (1).
Next, we give the proof of Proposition 1 based on (1) and (2).

\begin{mypro}{(Convergence rate of Algorithm 1)}
If $0\le\eta\le\frac{2(1-\beta)}{\mu+L}$,$0\le\alpha<1$,$0\le\beta=p\alpha<1$, then we obtain the convergence of $d_t$\\
\begin{equation}\label{eq:rate}
    \begin{split}
        d_{t}\le h^t d_0+(c_0-\frac{\eta^2\sigma_1^2}{\gamma})(1-\gamma)^t(1-(\frac{p}{p+1})^t)+\eta^2\sigma_1^2\frac{1-h^t}{\gamma},\\
        where\  0<h=\frac{p(1-\gamma)}{p+1}<1,k=\frac{1-\gamma}{p+1},\gamma=2\eta\frac{\mu L}{\mu+L}\\
        and\ c_0=\mathop{max}\limits_{i=1,...,p,f}\parallel w^i_0-w^*\parallel^2
    \end{split}
\end{equation}
\end{mypro}

\emph{Proof} From the sorting rule and the Assumption 5.1(2), we can easily obtain the inequality relation of $a_t$,$b_t$,$c_t$ and $d_t$
\begin{align}
    a_t\le d_t\le c_t\\
    and\ b_t\le d_t\le c_t
\end{align}
Applying (19) in (2), we have
\begin{equation}
    \begin{split}
         c_{t+1}\le(1-\gamma-\beta)c_t+\beta a_t+\eta^2\sigma_1^2\\
         \le(1-\gamma-\beta)c_t+\beta c_t+\eta^2\sigma_1^2\\
         =(1-\gamma)c_t+\eta^2\sigma_1^2
    \end{split}
\end{equation}
Through iterating this inequality with $t$, we have
\begin{equation}
    \begin{split}
         c_t\le(1-\gamma)^tc_0+\eta^2\sigma_1^2[1+(1-\gamma)+......+(1-\gamma)^t]\\
         =(1-\gamma)^tc_0+\eta^2\sigma_1^2\frac{1-(1-\gamma)^t}{\gamma}
    \end{split}
\end{equation}
Noting that $d_t=\frac{pb_t+c_t}{p+1}$ and use the (1),(2), we have
\begin{equation}
    \begin{split}
        d_t=\frac{pb_t+c_t}{p+1}\\
        \le\frac{p}{p+1}[(1-\gamma-\alpha)b_{t-1}+\alpha c_{t-1}+\eta^2\sigma_1^2]\\
        +\frac{1}{p+1}[\beta a_{t-1}+(1-\gamma-\alpha)c_{t-1}+\eta^2\sigma_1^2]\\
        =\frac{p(1-\gamma)}{p+1}d_{t-1}+\frac{1-\gamma}{p+1}c_{t-1}+\eta^2\sigma_1^2\\
        =h d_{t-1}+kc_{t-1}+\eta^2\sigma_1^2
    \end{split}
\end{equation}
Applying (20) in (21), we have
\begin{equation}
    \begin{split}
        d_t\le h d_{t-1}+k[(1-\gamma)^{t-1}c_0+\eta^2\sigma_1^2\frac{1-(1-\gamma)^{t-1}}{\gamma}]+\eta^2\sigma_1^2\\
        =h d_{t-1}+k(c_0-\frac{\eta^2\sigma_1^2}{\gamma})(1-\gamma)^{t-1}+(1+\frac{k}{\gamma})\eta^2\sigma_1^2
    \end{split}
\end{equation}
Through iterating this inequality with $t$, we have
\begin{equation}
    \begin{split}
        d_t\le h^t d_0+k(c_0-\frac{\eta^2\sigma_1^2}{\gamma})[(1-\gamma)^{t-1}+h(1-\gamma)^{t-2}+......+h^{t-1}]\\
        +(1+\frac{k}{\gamma})\eta^2\sigma_1^2[1+h+......+h^{t-1}]\\
        = h^t d_0+k(c_0-\frac{\eta^2\sigma_1^2}{\gamma})\frac{(1-\gamma)^t-h^t}{1-\gamma-h}+(1+\frac{k}{\gamma})\eta^2\sigma_1^2\frac{1-h^t}{1-h}
    \end{split}
\end{equation}
To simplify (25), we note that
\begin{align}
    k+h=1-\gamma\\
    \frac{1+\frac{k}{\gamma}}{1-h}=\frac{1+\frac{\frac{1-\gamma}{p+1}}{\gamma}}{1-\frac{p(1-\gamma)}{p+1}}\\
    =\frac{p+1+\frac{1-\gamma}{\gamma}}{p+1-p(1-\gamma)}\\
    =\frac{p+\frac{1}{\gamma}}{1+p\gamma}\\
    =\frac{1}{\gamma}
\end{align}
Hence, (25) can be rewriten as
\begin{equation}
    \begin{split}
         d_t\le h^t d_0+(c_0-\frac{\eta^2\sigma_1^2}{\gamma})[(1-\gamma)^t-h^t]+\frac{1}{\gamma}\eta^2\sigma_1^2(1-h^t)\\
         =h^t d_0+(c_0-\frac{\eta^2\sigma_1^2}{\gamma})(1-\gamma)^t(1-(\frac{p}{p+1})^t)+\eta^2\sigma_1^2\frac{1-h^t}{\gamma}
    \end{split}
\end{equation}
This concludes the proof.

\subsection{Comparison of convergence rate of LEASGD and DPSGD in the strongly-convex case}
We provide a proof to demonstrate the convergence rate of our LEASGD algorithm faster than that of DPSGD when $t \to \infty$.

\emph{Proof} Remember the two convergence rate of both algorithms is $O(1/[(p+1)t])$ and $O(h^t)$ respectively for DPSGD and LEASGD in the strongly-convex case. 
By dividing one with another, we have
\begin{equation}
    \begin{split}
        \frac{O(1/(p+1)t)}{O(h^t)}\\
        ={\lim_{t \to +\infty}} \frac{1/[(p+1)t]}{h^t}\\
        ={\lim_{t \to +\infty}} \frac{(1/h)^t}{(p+1)t}
    \end{split}
\end{equation}
Using L'Hospital's Rule and note $1/h>1$, we thus have
\begin{equation}
    \begin{split}
        {\lim_{t \to +\infty}} \frac{(1/h)^t}{(p+1)t}\\
        ={\lim_{t \to +\infty}} \frac{[(1/h)^t]'}{[(p+1)t]'}\\
        ={\lim_{t \to +\infty}} \frac{(1/h)^t ln(1/h)}{p+1}\\
        =\infty
    \end{split}
\end{equation}
This concludes proof. 



